Stein Points

An important task in computational statistics and machine learning is to approximate a posterior distribution $p(x)$ with an empirical measure supported on a set of representative points $\{x_i\}_{i=1}^n$. This paper focuses on methods where the selection of points is essentially deterministic, with an emphasis on achieving accurate approximation when $n$ is small. To this end, we present `Stein Points'. The idea is to exploit either a greedy or a conditional gradient method to iteratively minimise a kernel Stein discrepancy between the empirical measure and $p(x)$. Our empirical results demonstrate that Stein Points enable accurate approximation of the posterior at modest computational cost. In addition, theoretical results are provided to establish convergence of the method.

==> inverse_log_deriv_properties_proof.tex <==
%
\subsection{Proof of \lemref{inverse-log-gft-properties}: Integrability of
  Inverse Log Kernel Derivatives}

%
Before we are able to understand the integrability of $\Lap^m \Phi$ and
$\grad (\Lap^m \Phi)$, we will first need to prove an intermediate result via
induction. Suppose that for $m\in\mbb{N}_0$,
\begin{align}\label{eqn:lap-expansion}
\Lap^m \Phi(z) = \sum_{(u,v)\in S_m} \tau_{u,v} \twonorm{z}^{2v} \phi^{(u)}(\twonorm{z}^2)
\end{align}
where $\tau_{u,v} > 0$ are positive reals, $S_m = \{(u, v)\in\mbb{N}_0^2
\,\mid\, v\le u - m, u\le 2m\}$ and $\phi(r)\defeq (a + \log(g + r))^{-1}$.

Note for the base case $m=0$, the claim above for $\Lap^0 \Phi = \Phi$
clearly holds. Now suppose it holds from some $m\in\mbb{N}_0$.
If $A:\mbb{R}^d\to\mbb{R}$ is a function that can be written as
$A(z) \defeq f(\twonorm{z}^2)g(\twonorm{z}^2)$
where $f,g \in C^{\infty}([0,\infty))$, then we have
\begin{align}\label{eqn:laplacian-product-rule}
%
%
\Lap A(z)
  %
  %
  %
  %
  %
  &= \left [2d g'(\twonorm{z}^2) + 4\twonorm{z}^2 g''(\twonorm{z}^2)\right ]
  f(\twonorm{z}^2) +
  \left [2d g(\twonorm{z}^2) + 4\twonorm{z}^2 g'(\twonorm{z}^2)\right ]
  f'(\twonorm{z}^2) +
  4\twonorm{z}^2 g(\twonorm{z}^2) f''(\twonorm{z}^2).
\end{align}
Consider each term in the decomposition of $\Lap^m \Phi(z)$ from the induction
hypothesis. If we let $g(r) = r^{v}$ and $f(r) = \phi^{(u)}(r)$, we see that
each term from \eqnref{laplacian-product-rule} is of the form $\tau_{u,v}'
\twonorm{z}^{2v'} \phi^{(u')}(\twonorm{z}^2)$ where the values for $(u',
v')$ are $(u, v-1), (u, v-1), (u+1, v), (u+1, v), (u+2, v+1)$
respectively. Notice that when $v=0$ or $v=1$, the first or second
derivative of $g$ will be zero and these terms may disappear altogether. Thus all
these tuples will lie in $S_{m+1}$ for any $(u,v)\in S_m$, and so we must have
$\Lap^{m+1} \Phi(z)$ satisfies the induction hypothesis as well, completing
the proof by induction.

Using this result, we can take derivatives to infer
\begin{align*}
(\grad \Lap^m) \Phi(z) = \sum_{(u,v)\in T_m} \tau_{u,v} z \twonorm{z}^{2v} \phi^{(u)}(\twonorm{z}^2)
\end{align*}
where $T_m \defeq \{(u, v)\in\mbb{N}_0^2 \,\mid\, v\le u - m - 1, u\le 2m + 1\}$
and $\tau_{u,v}\in\mbb{R}$ are a different set of constants for all $m\in\mbb{N}_0$.

Now we can prove the various integrability conditions regarding the
derivatives of $\Phi$. We first will show that $\Lap^m \Phi \in
L^1(\mbb{R}^d)$ when $2m \ge d$.  Then by the triangle inequality and a
radial substitution \cite{Baker1999},
\begin{align*}
  \int_{\mbb{R}^d} |\Lap^m \Phi(z)|\dz
    \le \sum_{(u,v)\in S_m} \int_{\mbb{R}^d} \tau_{u,v} \twonorm{z}^{2v}
    |\phi^{(u)}(\twonorm{z}^2)| \dz
    = d V_d \sum_{(u,v)\in S_m} \int_{\mbb{R}^d} \tau_{u,v} r^{2v + d - 1}
    |\phi^{(u)}(r^2)| \dz,
\end{align*}
where $V_d$ is the volume of the unit Euclidean ball in $d$ dimensions.
Because $|\phi^{(u)}(r)| = O(r^{-u}\log^{-2}(r))$ for $u\in\mbb{N}$ by
\eqnref{inverse-log-radial-derivs}, we see that each term above is $O(r^{2(v-u)
  + d - 1} \log^{-2}(r))$. But since $v \le u - m$, this will imply that
each integrand is $O(r^{-2m + d - 1} \log^{-2}(r))$, which is integrable for
large $r$ whenever $d \le 2m$ yielding $\Lap^m \Phi \in L^1(\mbb{R}^d)$.

\jcg{TODO: Show when $\Lap^m \Phi$ is NOT in $L_2$...}


==> inverse_log_gft_properties_proof.tex <==
%
\subsection{Proof of \lemref{log-kernel-gft-properties}: Demonstration of
  Properies of Inverse Log GFT}

\begin{lemma}[Exponential Decay of Inverse Log
    GFT]\label{lem:exp-decay-inverse-log-gft}
Let $\Phi(z)\defeq (\alpha + \log(\gamma + \twonorm{z}^2))^{-1}$ be the
translation invariant inverse log kernel where $\gamma - e^{-\alpha} > 0$. Then
the generalized Fourier transform $\hat{\Phi}(\omega)$ decays exponentially
for large $\twonorm{\omega}$, i.e., $e^{v\twonorm{w}}\hat{\Phi}(\omega)\to 0$
as $\twonorm{\omega}\to\infty$ if and only if $v\in (0,(\gamma - e^{-\alpha})^{1/2})$.
\end{lemma}

For the duration of this proof, we will overload $\twonorm{z}^2 \defeq
\sum_{j=1}^d z_j^2$ whenever $z\in\mbb{C}^d$.
Let us extend the function $\Phi:\mbb{C}^d\to\mbb{C}^d$ to be the analytic
continuation of $\Phi$ that maps $z$ to $(\alpha + \log (\gamma +
\twonorm{z}^2))^{-1}$. We will utilize the notion of a strip
$\mathcal{S}_{\eta}\subseteq \mbb{C}^d$ defined as
$\mathcal{S}_{\eta}\defeq \{z\in\mbb{C}^d \,\mid\, \twonorm{\Im(z)} <
\eta\}$ for all $\eta > 0$. Our first step is to show
that $\Phi(z)$ is holomorphic on the strip $\mathcal{S}_{\eta}$ if and only
if $\eta < (\gamma - e^{-\alpha})^{1/2}$.

Because polynomials are holomorphic, we first note the function $z \mapsto g
+ \twonorm{z}^2$ is an entire function. Since the function $z \mapsto \log
z$ is holomorphic on the set $\mbb{C}^d\setminus \{-\gamma\in\mbb{R}\,\mid\, \gamma\ge 0\}$
and the composition of holomorphic functions is again holomorphic,
it is worth checking when $g + \twonorm{z}^2 = -\gamma$ for some real
$\gamma\ge 0$. Notice for $x,y\in\mbb{R}^d$, we have
\begin{align*}
  \twonorm{x+iy}^2 = \sum_{j=1}^d (x_j^2 - y_j^2) + 2x_j y_j i
  \Rightarrow \Re (\twonorm{x+iy}^2) \ge -\twonorm{y}^2.
\end{align*}
Thus $z\mapsto \log(\gamma + \twonorm{z}^2)$ is holomorphic on the strip
$\mathcal{S}_{\eta}$ if and only if $\eta \le \gamma^{1/2}$.

Finally, consider the function $z\mapsto \frac{1}{a + z}$. This function is
holomorphic for all $z\neq a$. Thus for $\Phi$ to be holomorphic on the
strip $\mathcal{S}_{\eta}$, we must have $\alpha + \log (\gamma + \eta^2) >
0$ which implies $|\eta| < (\gamma - e^{-\alpha})^{1/2}$. Since $(\gamma -
e^{-\alpha})^{1/2} < \gamma^{1/2}$ for all $\alpha$, we have that $\Phi$ is
holomorphic on the strip $\mathcal{S}_{\eta}$ if and only if $\eta < (\gamma -
e^{-\alpha})^{1/2}$ as desired.

Let us now consider the function $\Lap^m \Phi$ for some integral $m \ge
d/4$. Our goal will be to show that for any $y\in\mbb{R}^d$ such that
$\twonorm{y} < (\gamma - e^{-\alpha})^{1/2}$, the function $x\mapsto \Lap^m\Phi(x
+ iy)$ will belong to $L^2(\mbb{R}^d)$. Using \eqnref{lap-expansion} and the
triangle inequality, we see that for any fixed $y$,
\begin{align}\label{eqn:analytic-continuation-l2-bound}
\int_{\mbb{R}^d} \norm{\Lap^m\Phi(x + iy)}_{L^2}^2 \dx
  &= \int_{\mbb{R}^d} |\Lap^m\Phi(x + iy)| |\overline{\Lap^m\Phi(x + iy)}|
    \dx \notag \\
  &\le \int_{\mbb{R}^d} \left (\sum_{(k,l)\in S_m}
\tau_{k,l}|\twonorm{x+iy}^{2l}\phi^{(k)}(\twonorm{x+iy}^2)|\right )
\left (\sum_{(k',l')\in S_m}
\tau_{k',l'}|\twonorm{x+iy}^{2l'}\phi^{(k')}(\twonorm{x+iy}^2)|\right )
\dx \notag \\
  &= \int_{\mbb{R}^d} \sum_{\substack{(k,l)\in S_m \\ (k', l')\in S_m}}
  \tau_{k,l}\tau_{k',l'}\left |\twonorm{x+iy}^{2(l+l')}
    \phi^{(k)}(\twonorm{x+iy}^2) \phi^{(k')}(\twonorm{x+iy}^2)\right |
    \dx \notag \\
  &\le \int_{\mbb{R}^d} \sum_{\substack{(k,l)\in S_m \\ (k', l')\in S_m}}
    \tau_{k,l}\tau_{k',l'} (\twonorm{x}^2 + \twonorm{y}^2)^{l+l'}
    \left | \phi^{(k)}(\twonorm{x+iy}^2) \phi^{(k')}(\twonorm{x+iy}^2)\right |
    \dx.
\end{align}
We must now bound $|\phi^{(b)}(\twonorm{x+iy}^2)|$. Again using
\eqnref{inverse-log-radial-derivs} and the triangle inequality, we have
\begin{align*}
|\phi^{(b)}(\twonorm{x+iy}^2)| \le \sum_{a=2}^{b+1} c_{a,b} |\alpha +
\log(\gamma + \twonorm{x+iy}^2)|^{-a} |\gamma + \twonorm{x+iy}^2|^{-b}.
\end{align*}
Since we are assuming $\twonorm{y}^2 < \gamma$, this implies
$|\gamma + \twonorm{x+iy}^2| \ge \Re (\gamma + \twonorm{x+iy}^2) = \gamma
-\twonorm{y}^2 + \twonorm{x}^2$. Hence we have $|\gamma +
\twonorm{x+iy}^2|^{-b} \le (\gamma -\twonorm{y}^2 +
\twonorm{x}^2)^{-b}$. Moreover, this implies that $\Re(\log(\gamma +
\twonorm{x+iy}^2)) \ge \log (\gamma - \twonorm{y}^2 + \twonorm{x}^2)$ and
since we assume $\alpha + \log(\gamma + \twonorm{y}^2) > 0$ this implies
that $|\alpha + \log(\gamma + \twonorm{x+iy}^2)| \ge |\alpha + \log(\gamma -
\twonorm{y}^2 + \twonorm{x}^2)|$. This finally yields
\begin{align*}
|\phi^{(b)}(\twonorm{x+iy}^2)| \le
  \sum_{a=2}^{b+1} c_{a,b} |\alpha + \log(\gamma - \twonorm{y}^2 + \twonorm{x}^2)|^{-a}
  (\gamma -\twonorm{y}^2 + \twonorm{x}^2)^{-b}
\end{align*}
It follows that each term in \eqnref{analytic-continuation-l2-bound} is
$O(\twonorm{x}^{-4m} \log^{-2}(\twonorm{x})$, which implies the integral is
infinite. Moreover, for any $\eta < (\gamma - e^{-\alpha})^{1/2}$, we see
that $\norm{\Lap^m\Phi(x + iy)}_{L^2}$ is uniformly bounded for all
$\twonorm{y} < \eta$. This allows us to invoke the Paley-Wiener result
\citep[Theorem IX.13]{Reed1978} which implies that $\omega \mapsto
e^{v\twonorm{\omega}} \widehat{\Lap^m \Phi}(\omega)$ is in $L^2$ if and only if
$v < (\gamma - e^{-\alpha})^{1/2}$. \jcg{Yikes- is this enough?? We need to
  lower bound hat(Phi) for large w and this doesnt exactly do that}. In particular, since
$e^{v\twonorm{\omega}} \widehat{\Lap^m \Phi}(\omega) =
e^{v\twonorm{\omega}}\twonorm{w}^{2m} \hat{\Phi}(\omega)$ for all
$\omega\in\mbb{R}^d$, this shows us that $e^{v_0} \hat{\Phi}(\omega) \to 0$
as $\twonorm{\omega}\to\infty$ for any $v_0 \in (0, (\gamma -
e^{-\alpha})^{1/2})$ as desired.

